Meta Propagation Networks for Graph Few-shot Semi-supervised Learning

Inspired by the extensive success of deep learning, graph neural networks (GNNs) have been proposed to learn expressive node representations and demonstrated promising performance in various graph learning tasks. However, existing endeavors predominately focus on the conventional semi-supervised setting where relatively abundant gold-labeled nodes are provided. While it is often impractical due to the fact that data labeling is unbearably laborious and requires intensive domain knowledge, especially when considering the heterogeneity of graph-structured data. Under the few-shot semi-supervised setting, the performance of most of the existing GNNs is inevitably undermined by the overfitting and oversmoothing issues, largely owing to the shortage of labeled data. In this paper, we propose a decoupled network architecture equipped with a novel meta-learning algorithm to solve this problem. In essence, our framework Meta-PN infers high-quality pseudo labels on unlabeled nodes via a meta-learned label propagation strategy, which effectively augments the scarce labeled data while enabling large receptive fields during training. Extensive experiments demonstrate that our approach offers easy and substantial performance gains compared to existing techniques on various benchmark datasets.

==> 07Checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to %answer these
%questions.  For each question, change the default \answerTODO{} to %\answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a %{\bf
%justification to your answer}, either by referencing the appropriate %section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Section~\ref{sec:conclusion}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Please see the supplemental material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please see the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please see Section~\ref{sec:experiment} and the supplemental material}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{sec:experiment}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable? \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \answerNA{}
\end{enumerate}

\end{enumerate}

==> Preliminary.tex <==
%  \begin{figure}[t]
%     \graphicspath{{figures/}}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figures/GNN.pdf}
%     \caption{Illustration of the neighborhood aggregation scheme of graph neural networks.}%
%     \label{fig:agg_framework}%
% \end{figure}

To legibly describe the studied problem, we follow the commonly used notations throughout the paper. Specifically, we use lowercase letters to denote scalars 
% $\lambda$,
(e.g., $x$), boldface lowercase letters to denote vectors (e.g., $\mathbf{x}$), boldface uppercase letters to denote matrices (e.g., $\mathbf{X}$), and calligraphic fonts to denote sets (e.g., $\mathcal{V}$). 


We denote a graph as $G = (\mathcal{V}, \mathcal{E}, \mathbf{X})$, where $\mathcal V$ is the set of $n$ nodes and $\mathcal{E}$ is the set of $m$ edges. $\mathbf{X} = [\mathbf{x}_1, \mathbf{x}_2, \dots, \mathbf{x}_n] \in \mathbb{R}^{n \times d}$ denotes the features of these $n$ nodes. The $j^{th}$ feature value of node $i$ is denoted as $x_{ij}$. Commonly, the topological structure of a graph can be represented by the adjacency matrix $\mathbf{A} = \{0, 1\}^{n \times n}$, where $a_{ij}=1$ indicates that there is an edge between node $i$ and node $j$; otherwise, $a_{ij}=0$. Here we focus on undirected graphs, though it is straightforward to extend our approach to directed graphs. For other notations, we introduce them in later sections. Formally, our studied problem can be defined as:

\begin{problem}
\textbf{Feature Interaction-aware Node Representation Learning}: Given an input graph $G = (\mathbf{A}, \mathbf{X})$, the model objective is to map nodes $\mathcal{V}$ to latent representations $\mathbf{Z} = [\mathbf{z}_1, ..., \mathbf{z}_n] \in \mathbb{R}^{n \times d'}$, where each node representation $\mathbf{z}_i$ incorporates interactions between its features $\mathbf{x}_i$.
\end{problem} 



% \begin{table}[t]
%   \label{tab:symbols}
%   \caption{Table of main notations.}
%   \begin{tabular}{c|cl}
%     \toprule
%     Notations & Definitions \\
%     \midrule
%     $G = (\mathbf{X}, \mathbf{A})$ & input graph \\
  
%     % ${\mathbf X}$ & the attribute matrix \\
%     % ${\mathbf A}$ & the adjacency matrix \\
%     ${\mathbf W}$ & parameter matrix \\
%     $\mathbf{h} \in \mathbb{R}^k$ & embedding of aggregated features \\
%     $\mathbf{f} \in \mathbb{R}^k$ &  embedding of feature interactions \\
%     $\mathbf{z}$ & unified node representation \\

%     ${\mathbf x} \in \mathbb{R}^d$ & node attribute vector \\
%     ${\mathbf v} \in \mathbb{R}^k$ &  feature embedding vector \\

%     ${\mathcal N}_i$ & the neighbors of node $i$\\
%     ${n}$ & number of nodes \\
%     ${m}$ &  number of edges\\
%     ${d}$ &  dimension of node features \\
%     ${k}$ &  dimension of embedding vector \\
   
%     \bottomrule
    
%   \end{tabular}
% \end{table}



% \subsection{Factorization Machines}
% Factorization machines (FMs), an effective learning paradigm originally proposed in~\cite{rendle2010factorization}, have recently gained popularity for sparse data prediction. Specifically, given a real-valued feature vector $\mathbf{x} \in \mathbb{R}^d$, the vanilla FM estimates the target value by modeling all the interactions between each pair of features via factorized interaction parameters:
% \begin{equation}
%     y_{\text{FM}}(\mathbf{x}) =  \underbrace{w_0 + \sum_{i = 1}^{d}w_i x_i}_{\small \text{linear regression}} + \underbrace{\sum_{i = 1}^{d} \sum_{j = i+1}^{d}  \langle\mathbf{v}_i, \mathbf{v}_j\rangle  \cdot x_i x_j}_{\small \text{pair-wise feature factorization}},
%     \label{eq:1}%
% \end{equation}
% where $w_0$ is the global bias, $w_i$ is a parameter which models the weight of the $i$-th
% feature $x_i$ to the target. The feature interaction between feature $x_i$ and $x_j$ is captured by a factorized term $ \langle\mathbf{v}_i, \mathbf{v}_j\rangle$, where $\langle \cdot, \cdot \rangle$ denotes the inner product of two vectors. Here $\mathbf{v}_i \in \mathbb{R}^k$ denotes the $k$-dimensional embedding vector for feature $x_i$. In practice, only interactions of non-zero features will be considered in the computation. 

% Theoretically, FM enhances linear/logistic regression (LR) by incorporating the second-order factorized interactions between features, and has been successfully applied to many sparse predictive tasks, ranging from recommendation~\cite{rendle2010factorization}, search ranking~\cite{lu2017multilinear}, to relation extraction~\cite{petroni2015core}. In light of this, we try to enhance the expressive power of GNNs on feature-sparse graphs by leveraging the capability of FM.
% \JL{what about high-order interactions? FM is initially designed to capture high-order interactions}
% have recently gained
% popularity as an effective learning paradigm for capturing impact of feature conjunctions especially for sparse datasets

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> Rebuttal.tex <==
\section*{General Response}
We first thank all the reviewers for recognizing our work and giving constructive feedback! Here we summarize two main concerns from reviewers: (C1) why our model can address oversmoothing? and (C2) why we didn't compare with graph few-shot learning models? Our explanations are as follows:
\begin{itemize}[leftmargin=*,noitemsep,topsep=1.5pt]
    \item \textbf{C1.} As analyzed by previous research, there are two main factors causing the oversmoothing issue. First, aggregation by averaging makes the model lose its focus on the local neighborhood if too many layers are used, given the graph is irreducible and aperiodic. Second, the entanglement of representation transformation and propagation makes the number of parameters in transformation intertwined with the receptive fields in propagation. Therefore, using a larger neighborhood necessarily increases the depth and number of learnable parameters of the neural network, which further magnifies the difficulty of learning discriminative node representations. Our model adopts a decoupled design that performs label propagation and feature transformation separately. By removing the entanglement of representation transformation and propagation, we can leverage large receptive fields without introducing a lot more trainable parameters. Moreover, based on the proposed meta-learning algorithm, the label propagator in our framework is able to adaptively adjust the contributions of different receptive fields by learning with only a few labels. This way the model can capture both the local and global structural information while avoiding the oversmoothing issue.
    
    
    % This global property is therefore unsuitable for describing the root node’s neighborhood, 
    
    
    % most common aggregation schemes use learnable weight matrices in each layer. T
   
    
    % (More theoretical analysis can be found in the paper of DAGNN)
    
    
    \item \textbf{C2.} It is worth mentioning that \textit{few-shot learning} and \textit{few-shot semi-supervised learning} are two different learning paradigms. In general, a few-shot learning model aims to classify instances in a set of \textit{unseen} classes by transferring the knowledge from a disjoint set of \textit{seen} classes. Thus graph few-shot learning methods require an auxiliary (meta-training) dataset that has abundant labeled nodes from those seen node classes. In contrast, our problem focuses on a more practical scenario where no auxiliary dataset is available, and that’s why we didn't include graph few-shot learning methods in our comparisons since they cannot be applied to our problem. In essence, the problem we try to solve is a semi-supervised node classification problem where each class only has a few labeled nodes. The key to solving this problem is how to effectively leverage unlabeled nodes to augment the scarce labeled training data, also how to enable large receptive fields for better propagation of label signals.
    
    % Different from graph few-shot learning models that require to transfer the knowledge from seen classes to unseen classes, we try to solve the few-shot semi-supervised node classification problem by 
    
    %  (as discussed in our Introduction)
    
    
    % As we mentioned in our introduction, under the low-resource setting, the GNN model needs more propagation steps to propagate the information from labeled nodes to unlabeled nodes. On the contrary, label propagation can enable more propagation steps without losing the focus on the local neighborhood. 
    
    
    %   learns across diverse meta-training tasks sampled from those seen classes with a large quantity of labeled data, and tries to transfer the meta-knowledge to new tasks (i.e., meta-test task) from unseen classes during training. 

\end{itemize}

\section*{Response to Reviewer 1}

\noindent\textbf{Q1: Few-shot graph learning.} As we mentioned in the paper, graph few-shot learning methods are inherently inapplicable for the (few-shot) semi-supervised node classification task since they require an auxiliary dataset that contains a large amounts of labeled nodes. More detailed discussions can be found in our general response C2. 

\noindent\textbf{Q2: Model design novelty.} Notably, previous works have not explicitly explored how to advance the decoupled modeling to solve few-shot semi-supervised learning problems. For example, the baseline C\&S~[1] uses 54\% labeled nodes for achieving good performance on the ogbn-arxiv dataset and performs badly in our evaluation. On the contrary, our approach leverages meta-learning to adaptively adjust the contribution of different receptive fields according to the model feedback on the labeled nodes, which not only enables better propagation of label signals, but also exerts the potential power of unlabeled data.

% Though decoupled modeling of label propagation and feature transformation has been proposed in the community, but


% In addition, [1,2] both use a disentangled modeling of label propagation and feature, and [2] also uses pseudo labels for modeling. More discussions or comparisons are needed.






\section*{Response to Reviewer 2}
\textbf{Q1: Few-shot results on ogbn.} In our experiments, we didn’t include the 3-shot and 5-shot results on the ogbn-arxiv dataset since the task on this this dataset is much harder (169K nodes, 40 node classes, with noisy structure) than other datasets. To better show the performance of different models, we conduct the evaluation with different label ratios (1.0\%, 1.5\%, 2.0\%, 2.5\%), as reported in our Figure 2. 

% If each class is only provided with 3 or 5 labeled nodes, all the model have similar poor performance.

\section*{Response to Reviewer 3}
\textbf{Q1: Oversmoothing.} Our proposed model decouples representation transformation from propagation and utilizes learnable scores to adaptively adjust the information from local and global neighborhoods. Though trained with only few labels, our model is able to learn discriminative representations without suffering the oversmoothing issue. Please refer to the general response (C1) for detailed explanation.


\noindent\textbf{Q2: Meta-GNNs.} As pointed out in our Introduction, either graph few-shot learning or cross-network transfer learning methods relies on auxiliary dataset to enable knowledge transfer. However, in the few-shot semi-supervised setting such auxiliary data source is not accessible, thus those models cannot be trained and tested. Here we focus on leveraging large receptive fields and unlabeled nodes. Please refer to our general response (C2) for detailed explanation.
	


\section*{Response to Reviewer 4}
\textbf{Q1:Parameter \& Ablation.} The parameter \& ablation study is mainly designed for evaluating our approach. For the two baselines we compared, GCN belongs to the first category (vanilla GNNs) baselines and Static-LP is an instantiation of the third category baselines (deep GNNs). For the models in the second category, as they usually perform worse than the third category models due to the incapability of handling the oversmoothing issue (same as vanilla GNNs), so here we omit this category in the comparisons.
	
\section*{Response to Reviewer 5}

\noindent\textbf{Q1: Meta-learning.} By using the proposed meta-learning algorithm, the adaptive label propagator is able to adjust the information from both local and global neighborhoods and make the unlabeled data have the aligned usage with labeled data by connecting the meta-learner and the target model. 


% How does the new meta-learning setup change the picture theoretically?
	
\noindent\textbf{Q2: Optimal pseudo labels.} The meta-learning objective of our approach is to infer ``optimal'' pseudo labels, but we are not guaranteed to always have the optimal solution since we use approximation in the bi-level optimization process. In this work we do not focus on how to avoid local optimal in bi-level optimization problems (a series of related works have been proposed) and we would like to replace this word.

